Dense Matchers for Dense Tracking

Optical flow is a useful input for various applications, including 3D reconstruction, pose estimation, tracking, and structure-from-motion. Despite its utility, the field of dense long-term tracking, especially over wide baselines, has not been extensively explored. This paper extends the concept of combining multiple optical flows over logarithmically spaced intervals as proposed by MFT. We demonstrate the compatibility of MFT with different optical flow networks, yielding results that surpass their individual performance. Moreover, we present a simple yet effective combination of these networks within the MFT framework. This approach proves to be competitive with more sophisticated, non-causal methods in terms of position prediction accuracy, highlighting the potential of MFT in enhancing long-term tracking applications.

==> tables/MFT_better_than_baselines_strided.tex <==
\begin{center}
\begin{tabular}{llrrrrrrrrrr}
base & method & AJ & < thrs & OA & vis prec & vis recall & < 1 & < 2 & < 4 & < 8 & < 16\\
\hline
RAFT & direct & 47.9 & 58.0 & 76.3 & 93.5 & 71.5 & 36.6 & 51.8 & 61.8 & 67.7 & 72.1\\
RAFT & chain & 49.4 & 62.3 & 80.9 & 90.9 & 81.1 & 33.6 & 52.6 & 67.8 & 76.5 & 80.9\\
RAFT & MFT & 56.3 & 71.0 & 86.9 & 88.8 & 92.4 & 41.2 & 63.4 & 78.1 & 84.7 & 87.7\\
\hline
DKM & chain & 38.6 & 70.7 & 57.3 & 95.9 & 44.8 & 46.8 & 65.2 & 76.1 & 81.3 & 84.2\\
DKM & direct & 43.9 & 67.2 & 62.1 & 95.0 & 51.9 & 46.0 & 62.0 & 71.5 & 76.5 & 80.1\\
DKM & MFT & 56.2 & 75.9 & 77.4 & 88.9 & 77.1 & 51.9 & 71.2 & 81.8 & 86.1 & 88.5\\
\hline
RoMa & direct & 47.2 & 70.1 & 66.9 & 92.7 & 59.8 & 45.6 & 62.9 & 74.5 & 81.6 & 85.6\\
RoMa & chain & 51.2 & 71.0 & 69.7 & 94.4 & 62.1 & 46.8 & 64.6 & 76.2 & 82.3 & 85.1\\
RoMa & MFT & 58.0 & 77.2 & 80.5 & 85.7 & 86.4 & 51.6 & 71.3 & 83.1 & 88.6 & 91.5\\
\end{tabular}
\end{center}

==> tables/ensemble_strided.tex <==
\begin{center}
\begin{tabular}{llrrrrrrrrrr}
position MFT                 & occlusion MFT & AJ   & < thrs & OA   & vis prec & vis recall & < 1  & < 2  & < 4  & < 8  & < 16 \\
\hline
RAFT                         & RAFT          & 56.3 & 71.0   & 86.9 & 88.8     & 92.4       & 41.2 & 63.4 & 78.1 & 84.7 & 87.7 \\
RoMa                         & RoMa          & 58.0 & 77.2   & 80.5 & 85.7     & 86.4       & 51.6 & 71.3 & 83.1 & 88.6 & 91.5 \\
RoMa                         & RAFT          & 60.6 & 77.2   & 86.9 & 88.8     & 92.4       & 51.6 & 71.3 & 83.1 & 88.6 & 91.5 \\
RoMa if confident, else RAFT & RAFT          & 61.7 & 77.7   & 86.9 & 88.8     & 92.4       & 51.7 & 71.8 & 83.8 & 89.2 & 91.8 \\
\end{tabular}
\end{center}
